Coverage-aware and Reinforcement Learning Using Multi-agent Approach for HD Map QoS in a Realistic Environment

One effective way to optimize the offloading process is by minimizing the transmission time. This is particularly true in a Vehicular Adhoc Network (VANET) where vehicles frequently download and upload High-definition (HD) map data which requires constant updates. This implies that latency and throughput requirements must be guaranteed by the wireless system. To achieve this, adjustable contention windows (CW) allocation strategies in the standard IEEE802.11p have been explored by numerous researchers. Nevertheless, their implementations demand alterations to the existing standard which is not always desirable. To address this issue, we proposed a Q-Learning algorithm that operates at the application layer. Moreover, it could be deployed in any wireless network thereby mitigating the compatibility issues. The solution has demonstrated a better network performance with relatively fewer optimization requirements as compared to the Deep Q Network (DQN) and Actor-Critic algorithms. The same is observed while evaluating the model in a multi-agent setup showing higher performance compared to the single-agent setup.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/Jeff.jpg}}]{Jeffrey Redondo} is a PhD. candidate in Computer Science at Northumbria University, UK. He has received the B.E.E degree from La Universidad Del Norte, Barranquilla, Colombia, in 2011, the M.S. degree from Tallinn University of Technology, Estonia, in 2019. He is participating in the research group Cyber Security and Network Systems (CyberNets) at Northumbria University, UK. His research interest includes evaluating the benefits of using machine learning to improve the quality of service in wireless technologies for autonomous vehicles.  
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/zhenhui.jpg}}]
{Zhenhui Yuan} is an Assistant Professor at the University of Warwick, UK. He received his B.Eng degree in Software Engineering at Wuhan University, China, in 2008 and PhD in Electronic Engineering at Dublin City University, Ireland, in 2012. He is primarily interested in the development of communication systems for robots and vehicles. He was a postdoctoral researcher at Ericsson and Enterprise Ireland and a visiting scholar at UCLA, U.S. He was also a 5G Senior Researcher at Huawei (Shanghai). He co-founded RobSense (Hangzhou) Technology Co.Ltd which provides industrial IoT solutions with robotics. He was an Associate Professor at Hangzhou Dianzi University, China, and a Senior Lecturer at Northumbria University, UK. He won the best paper awards at IEEE ICCRE 2016 and IEEE BMSB 2014. He served as the Lead Guest Editor in IEEE Network and IEEE Internet of Things Journal, and an Associate Editor at IEEE ACCESS, IEEE Transactions on Consumer Electronics and Journal of Pervasive Computing \& Communications. He is the founding chair of VeSUS (6G-empowered Robotic Vehicles for Sustainable Development) workshop. He is a voting member of IEEE P1954 on UAV communications.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/Nauman.jpg}}]
{Nauman Aslam} is a Professor in the Department of Computer and Information Science at Northumbria University, UK. He received his PhD in Engineering Mathematics from Dalhousie University, Canada in 2008. His research interests cover diverse but interconnected areas related to communication networks. His current research efforts are focused at addressing challenges related to Internet of Things (IoT), network security, charging management of electric vehicles and application of Artificial Intelligence (AI) in communication networks. He has held several grants as PI and CoI, from European Commission, EPSRC, Innovate UK and industry. He has co-authored over 200 peer-reviewed publications. He is the chair of IEEE UK and Ireland Communications Society (ComSoc) chapter.
\end{IEEEbiography}
